Property-based Polynomial Invariant Generation using Sums-of-Squares Optimization

While abstract interpretation is not theoretically restricted to specific kinds of properties, it is, in practice, mainly developed to compute linear over-approximations of reachable sets, aka. the collecting semantics of the program. The verification of user-provided properties is not easily compatible with the usual forward fixpoint computation using numerical abstract domains. We propose here to rely on sums-of-squares programming to characterize a property-driven polynomial invariant. This invariant generation can be guided by either boundedness, or in contrary, a given zone of the state space to avoid. While the target property is not necessarily inductive with respect to the program semantics, our method identifies a stronger inductive polynomial invariant using numerical optimization. Our method applies to a wide set of programs: a main while loop composed of a disjunction (if-then-else) of polynomial updates e.g. piecewise polynomial controllers. It has been evaluated on various programs.

==> erased.tex <==
\if{
For a given $m \in \nn$, let $(p_m,w_m) \in \rr_{2 m}[x] \times \rr$ be any feasible solution of Problem~\eqref{polsynthesis} and define the associated sublevel set $P_m := \{x \in \rr^d \mid p_m(x) \leq 0\}$.
Since $\Sigma[x]$ is a subset of positive polynomials then the sublevel sets $P_m$ and $\prop{\kappa, w_m}$ provide a solution of Problem~\eqref{eq:invsufficient}. We formulate this result as the following proposition:
}\fi
\if{
which satisfies $w_m \leq \alpha$.
guarantees that $P_m := {x \in \rd \mid p_m(x) \leq 0} \subseteq$. Assuming that $w_m \leq \alpha$, 
Since $\Sigma[x]$ is a subset of positive polynomials then a solution $(p_m,w_m) \in \rr_{2 m}[x] \times \rr$ of Problem~\eqref{polsynthesis} provides a solution of Problem~\eqref{eq:invsufficient} together with SOS certificates which guarantee that $P_m \subseteq \prop{\kappa, \alpha}$. 
We formulate this result as the following theorem:
%
\begin{proposition}
\label{fundamentalth}
Every feasible solution $(p,w)$ of Problem~\eqref{polsynthesis} is also a feasible solution of Problem~\eqref{eq:invsufficient}.
\end{proposition}
%Theorem~\ref{fundamentalth} uses the following lemma:
\begin{proof}%[SOS S-Lemma]
\label{funslemma}
%
Let $h,g_1,\ldots,g_n \in \rr[x]$.
If there exists $\mu\in \Sigma[x]^n$ such that
\[
\sum_{i=1}^n \mu_i(x)g_i(x))-h(x)\in\Sigma[x]\enspace ,
\]
then 
\[
\forall x \in \rd \, , (g_1(x)\leq 0\wedge \ldots\wedge g_n(x)\leq 0 \implies h(x)\leq 0) \, .
\]
\end{proof}
}\fi
